Neural Variational Learning for Grounded Language Acquisition

We propose a learning system in which language is grounded in visual percepts without specific pre-defined categories of terms. We present a unified generative method to acquire a shared semantic/visual embedding that enables the learning of language about a wide range of real-world objects. We evaluate the efficacy of this learning by predicting the semantics of objects and comparing the performance with neural and non-neural inputs. We show that this generative approach exhibits promising results in language grounding without pre-specifying visual categories under low resource settings. Our experiments demonstrate that this approach is generalizable to multilingual, highly varied datasets.

==> Makefile <==
NAME=main

.PHONY: all clean

all:

# We store all the auxiliary files tex creates in a separate build_dir
BUILDDICT=build_dir
WHERE=-output-directory=${BUILDDICT}

TEX=latexmk
TEX_FLAGS=-pdf -bibtex-cond

SECTIONS=$(filter-out $(NAME).tex, \
	$(shell find . -type f -name '*.tex') )

all: $(SECTIONS)
	@mkdir -p ${BUILDDICT} $(BUILDDICT)/tex
	${TEX} $(WHERE) $(TEX_FLAGS) $(NAME).tex
	@if [ -e "${BUILDDICT}/${NAME}.pdf" ]; then mv ${BUILDDICT}/${NAME}.pdf .; \
	echo "\n\n**************************" && \
	echo "Please see ${NAME}.pdf for final PDF output." && \
	echo "**************************"; \
	fi

.PHONY:list-sources
list-sources:
	@echo $(SECTIONS)

clean:
	@if [ -d ${BUILDDICT} ]; then rm -rf ${BUILDDICT}; rm -f ${NAME}.pdf; fi

clean-backup:
	find . -type f -name '*~' -delete

.PHONY: push pull
push:
	git push origin master

pull:
	git pull origin master


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
